A Novel Unsupervised Post-Processing Calibration Method for DNNS with Robustness to Domain Shift

The uncertainty estimation is critical in real-world decision making applications, especially when distributional shift between the training and test data are prevalent. Many calibration methods in the literature have been proposed to improve the predictive uncertainty of DNNs which are generally not well-calibrated. However, none of them is specifically designed to work properly under domain shift condition. In this paper, we propose Unsupervised Temperature Scaling (UTS) as a robust calibration method to domain shift. It exploits unlabeled test samples instead of the training one to adjust the uncertainty prediction of deep models towards the test distribution. UTS utilizes a novel loss function, weighted NLL, which allows unsupervised calibration. We evaluate UTS on a wide range of model-datasets to show the possibility of calibration without labels and demonstrate the robustness of UTS compared to other methods (e.g., TS, MC-dropout, SVI, ensembles) in shifted domains.

==> Table/table_nll_acc.tex <==
\begin{table}[t]
\begin{center}
\caption{NLL$\downarrow$ for UTS and other post-processing approaches for the training and test domains with the same distribution. In all cases UTS can calibrate the model without labeled samples, however it does not achieve the best results. The mean and std are reported in $20$ independent runs.}\label{table:nll_acc}
\vspace{-0.3cm}
\resizebox{\textwidth}{!}{ 
\begin{tabular}{llcccccccc}
\hline
\textbf{}        & \textbf{}                           & \multicolumn{3}{c}{\textbf{Accuracy (\%)}}                                                                        & \multicolumn{5}{c}{\textbf{Negative log-likelihood}}                                                                                                                      \\
\textbf{Dataset} & \textbf{Model}                      & \multicolumn{1}{l}{\textbf{UNC, TS, ATS}} & \multicolumn{1}{l}{\textbf{VS}} & \multicolumn{1}{l}{\textbf{MS}}     & \multicolumn{1}{l}{\textbf{UNC}} & \multicolumn{1}{l}{\textbf{TS}} & \multicolumn{1}{l}{\textbf{UTS}} & \multicolumn{1}{l}{\textbf{VS}} & \multicolumn{1}{l}{\textbf{MS}} \\ \hline
Birds            & \multicolumn{1}{l|}{ResNet50}       & \textbf{76.03}                            & 75.94                           & \multicolumn{1}{c|}{38.82}          & 0.9383                           & \textbf{0.9287}                 & 0.9313                           & 0.9355                          & 7.1423                          \\
MNIST            & \multicolumn{1}{l|}{Lenet-5}        & \textbf{99.19}                            & 99.18                           & \multicolumn{1}{c|}{99.11}          & 0.1044                           & \textbf{0.0243}                 & 0.0429                           & 0.0988                          & 0.1187                          \\
SVHN             & \multicolumn{1}{l|}{ResNet110}      & \textbf{96.09}                            & 96.07                           & \multicolumn{1}{c|}{96.08}          & 0.2107                           & \textbf{0.1534}                 & 0.1566                           & 0.1936                          & 0.2070                          \\
SVHN             & \multicolumn{1}{l|}{DenseNet100}    & 95.77                                     & \textbf{95.94}                  & \multicolumn{1}{c|}{95.86}          & 0.1803                           & \textbf{0.1608}                 & 0.1735                           & 0.1687                          & 0.1754                          \\
CIFAR10          & \multicolumn{1}{l|}{DenseNet40}     & \textbf{92.67}                            & 92.20                           & \multicolumn{1}{c|}{92.55}          & 0.2895                           & \textbf{0.2221}                 & 0.2848                           & 0.2912                          & 0.2883                          \\
CIFAR10          & \multicolumn{1}{l|}{DenseNet100}    & \textbf{95.08}                            & 94.81                           & \multicolumn{1}{c|}{95.02}          & 0.1973                           & \textbf{0.1559}                 & 0.1635                           & 0.2006                          & 0.1965                          \\
CIFAR10          & \multicolumn{1}{l|}{ResNet110}      & \textbf{93.62}                            & 93.53                           & \multicolumn{1}{c|}{93.49}          & 0.3134                           & \textbf{0.2069}                 & 0.2341                           & 0.2907                          & 0.3103                          \\
CIFAR10          & \multicolumn{1}{l|}{VGG16}          & 93.38                                     & 93.39                           & \multicolumn{1}{c|}{\textbf{93.40}} & 0.2608                           & \textbf{0.2036}                 & 0.2099                           & 0.2503                          & 0.2573                          \\
CIFAR100         & \multicolumn{1}{l|}{DenseNet40}     & \textbf{71.56}                            & 66.89                           & \multicolumn{1}{c|}{63.79}          & 1.0964                           & \textbf{1.0064}                 & 1.0217                           & 1.2876                          & 1.4914                          \\
CIFAR100         & \multicolumn{1}{l|}{DenseNet100}    & \textbf{75.87}                            & 73.38                           & \multicolumn{1}{c|}{73.12}          & 1.1285                           & \textbf{0.8751}                 & 0.8889                           & 1.2470                          & 1.2761                          \\
CIFAR100         & \multicolumn{1}{l|}{ResNet110}      & \textbf{70.41}                            & 67.24                           & \multicolumn{1}{c|}{65.27}          & 1.2442                           & \textbf{1.0466}                 & 1.0636                           & 1.3869                          & 1.5358                          \\
CIFAR100         & \multicolumn{1}{l|}{WideResNet40-4} & \textbf{79.80}                            & 79.57                           & \multicolumn{1}{c|}{79.79}          & 0.8751                           & \textbf{0.8192}                 & 0.8439                           & 0.8757                          & 0.8609                          \\ \hline
\end{tabular}
}
\end{center}
\end{table}

==> TableFiles/table_acc_nll.tex <==
\begin{table}[t]
\label{table1}
\begin{center}
\caption{Comparing UTS with other post-processing approaches for the training and test domains with the same distribution. In all cases UTS can calibrate the model without labeled samples, however it does not achieve the best results. All the experiments are repeated $20$ times and mean and std are reported. UNC = Uncalibrated, MS= Matrix Scaling, VS = Vector Scaling, TS= Temperature Scaling, UTS= Unsupervised Temperature Scaling  }
\resizebox{\textwidth}{!}{  
\begin{tabular}{llllllllll}
\hline
\textbf{}        & \textbf{}                           & \multicolumn{3}{c}{\textbf{Accuracy (\%) $\uparrow$}}                                                       & \multicolumn{5}{c}{\textbf{NLL$\downarrow$}}                                                       \\
\textbf{Dataset} & \textbf{Model}                      & \textbf{UNC, TS, UTS}   & \textbf{VS}             & \textbf{MS}                                  & \textbf{UNC}      & \textbf{TS}                & \textbf{UTS}      & \textbf{VS}       & \textbf{MS}       \\ \hline
Birds            & \multicolumn{1}{l|}{ResNet50}       & \textbf{76.03 +/- 0.17} & 75.94 +/- 0.31          & \multicolumn{1}{l|}{38.82 +/- 1.92}          & 0.9383 +/- 0.0086 & \textbf{0.9287 +/- 0.0077} & 0.9313 +/- 0.0078 & 0.9355 +/- 0.0093 & 7.1423 +/- 0.2424 \\
MNIST            & \multicolumn{1}{l|}{Lenet-5}        & \textbf{99.19 +/- 0.03} & 99.18 +/- 0.03          & \multicolumn{1}{l|}{99.11 +/- 0.05}          & 0.1044 +/- 0.0064 & \textbf{0.0243 +/- 0.0013} & 0.0429 +/- 0.0009 & 0.0988 +/- 0.0073 & 0.1187 +/- 0.0094 \\
SVHN             & \multicolumn{1}{l|}{ResNet110}      & \textbf{96.09 +/- 0.08} & 96.07 +/- 0.08          & \multicolumn{1}{l|}{96.08 +/- 0.08}          & 0.2107 +/- 0.0035 & \textbf{0.1534 +/- 0.0023} & 0.1566 +/- 0.0030 & 0.1936 +/- 0.0035 & 0.2070 +/- 0.0036 \\
SVHN             & \multicolumn{1}{l|}{DenseNet100}    & 95.77 +/- 0.03          & \textbf{95.94 +/- 0.02} & \multicolumn{1}{l|}{95.86 +/- 0.02}          & 0.1803 +/- 0.0017 & \textbf{0.1608 +/- 0.0013} & 0.1735 +/- 0.0048 & 0.1687 +/- 0.0025 & 0.1754 +/- 0.0017 \\
CIFAR10          & \multicolumn{1}{l|}{DenseNet40}     & \textbf{92.67 +/- 0.12} & 92.20 +/- 0.10          & \multicolumn{1}{l|}{92.55 +/- 0.04}          & 0.2895 +/- 0.0058 & \textbf{0.2221 +/- 0.0034} & 0.2848 +/- 0.0419 & 0.2912 +/- 0.0076 & 0.2883 +/- 0.0061 \\
CIFAR10          & \multicolumn{1}{l|}{DenseNet100}    & \textbf{95.08 +/- 0.09} & 94.81 +/- 0.12          & \multicolumn{1}{l|}{95.02 +/- 0.11}          & 0.1973 +/- 0.0060 & \textbf{0.1559 +/- 0.0035} & 0.1635 +/- 0.0051 & 0.2006 +/- 0.0098 & 0.1965 +/- 0.0061 \\
CIFAR10          & \multicolumn{1}{l|}{ResNet110}      & \textbf{93.62 +/- 0.13} & 93.53 +/- 0.14          & \multicolumn{1}{l|}{93.49 +/- 0.13}          & 0.3134 +/- 0.0083 & \textbf{0.2069 +/- 0.0047} & 0.2341 +/- 0.0109 & 0.2907 +/- 0.0090 & 0.3103 +/- 0.0081 \\
CIFAR10          & \multicolumn{1}{l|}{VGG16}          & 93.38 +/- 0.12          & 93.39 +/- 0.14          & \multicolumn{1}{l|}{\textbf{93.40 +/- 0.11}} & 0.2608 +/- 0.0060 & \textbf{0.2036 +/- 0.0039} & 0.2099 +/- 0.0065 & 0.2503 +/- 0.0093 & 0.2573 +/- 0.0064 \\
CIFAR100         & \multicolumn{1}{l|}{DenseNet40}     & \textbf{71.56 +/- 0.18} & 66.89 +/- 0.56          & \multicolumn{1}{l|}{63.79 +/- 0.81}          & 1.0964 +/- 0.0067 & \textbf{1.0064 +/- 0.0053} & 1.0217 +/- 0.0053 & 1.2876 +/- 0.0215 & 1.4914 +/- 0.0520 \\
CIFAR100         & \multicolumn{1}{l|}{DenseNet100}    & \textbf{75.87 +/- 0.15} & 73.38 +/- 0.25          & \multicolumn{1}{l|}{73.12 +/- 0.15}          & 1.1285 +/- 0.0072 & \textbf{0.8751 +/- 0.0042} & 0.8889 +/- 0.0054 & 1.2470 +/- 0.0186 & 1.2761 +/- 0.0129 \\
CIFAR100         & \multicolumn{1}{l|}{ResNet110}      & \textbf{70.41 +/- 0.26} & 67.24 +/- 0.20          & \multicolumn{1}{l|}{65.27 +/- 0.28}          & 1.2442 +/- 0.0132 & \textbf{1.0466 +/- 0.0090} & 1.0636 +/- 0.0140 & 1.3869 +/- 0.0186 & 1.5358 +/- 0.0204 \\
CIFAR100         & \multicolumn{1}{l|}{WideResNet40-4} & \textbf{79.80 +/- 0.22} & 79.57 +/- 0.15          & \multicolumn{1}{l|}{79.79 +/- 0.17}          & 0.8751 +/- 0.0111 & \textbf{0.8192 +/- 0.0096} & 0.8439 +/- 0.0089 & 0.8757 +/- 0.0095 & 0.8609 +/- 0.0103 \\ \hline
\end{tabular}
}
\end{center}

\end{table}
